The Robust Manifold Defense: Adversarial Training using Generative Models

We propose a new type of attack for finding adversarial examples for image classifiers. Our method exploits spanners, i.e. deep neural networks whose input space is low-dimensional and whose output range approximates the set of images of interest. Spanners may be generators of GANs or decoders of VAEs. The key idea in our attack is to search over latent code pairs to find ones that generate nearby images with different classifier outputs. We argue that our attack is stronger than searching over perturbations of real images. Moreover, we show that our stronger attack can be used to reduce the accuracy of Defense-GAN to 3\%, resolving an open problem from the well-known paper by Athalye et al. We combine our attack with normal adversarial training to obtain the most robust known MNIST classifier, significantly improving the state of the art against PGD attacks. Our formulation involves solving a min-max problem, where the min player sets the parameters of the classifier and the max player is running our attack, and is thus searching for adversarial examples in the {\em low-dimensional} input space of the spanner. All code and models are available at \url{https://github.com/ajiljalal/manifold-defense.git}

==> defenseGAN.tex <==
\paragraph{Circumventing DefenseGAN~\cite{samangouei2018defensegan}} 
DefenseGAN~\cite{samangouei2018defensegan} is a proposed adversarial defense technique that functions like our preliminary INC classifier.\citet{athalye2018obfuscated} show that by using an attack known as Backwards-Pass Differentiable Approximation (BPDA), it is possible to reduce the adversarial accuracy of DefenseGAN from the claimed 96\% accuracy to 55\% accuracy. This attack was completed under an $\ell_2$ threat model with an $\ell_2$ per-pixel distortion budget of $0.005$. Lowering the adversarial accuracy of DefenseGAN from 55\% to 0\% is posed as an open problem by~\citet{athalye2018obfuscated}.

By combining the latent-space attack that we propose in this work with the expectation-over-transformation attack of~\cite{athalye2017synthesizing}, we can successfully reduce the classification accuracy of DefenseGAN to \textbf{3\%}, under the same perturbation budget. In addition to resolving a major open problem, this attack demonstrates the potential of the latent-space attack as a more powerful attack for adversarial training.

 \paragraph{Generating new examples for~\citet{madry2017towards}}
  We also study the behavior of our proposed overpowered attack on the robust optimization-based defense (henceforth RO) of~\citet{madry2017towards}. Recall that this defense is given by solving the following min-max problem in input space:
% \begin{equation}
% \label{eq:robustopt}
% \min_\theta \mathbb{E}_{(x, y)\sim \mathcal{D}}\left[\max_\delta L_\theta(x+\delta, y)\right],
% \end{equation}

% exploiting Dantzig's theorem to find $\theta$ above with alternating gradient descent.

% The RO defense has proved to be one of the most robust adversarial defenses. Under an $\ell_2$ threat model with $\epsilon = 1.5$, the~\citet{madry2017towards} model is vulnerable to only 10\% of the MNIST test set. While this is a favorable outcome for robustntess, the size of the test set limits our ability to study the adversarial attacks which fool the model. It turns out, however, that the overpowered attack can be slightly adapted to generate significantly more adversarial examples against the~\citet{madry2017towards} defense. In particular, we use a variational autoencoder (VAE) as our spanning model. For any input $x$, we solve the following min-max attack problem:
% \begin{align}
% \inf_{\lambda \leq 0}\ \sup_{z}\ \  & L_\theta(d(z)) + 
% \lambda \cdot \left(\left|\left|{d(z) - d(e(x))}^2 - \eta\right|\right|\right)^2,
% \end{align}

% where $d$ and $e$ are the decoding and encoding functions of the VAE, respectively, and $L_\theta$ is the cross-entropy loss function for the classifier. Note that mounting this attack yields pairs of images in the range of the VAE---one of these images is $d(e(x))$ and is thus guaranteed to lay close to the original image $x$, and the other is found via latent-space optimization. By mounting this attack on the RO defense, we are able to generate new adversarial examples for \textbf{25\%} of the MNIST test set.\footnote{We point out that this does not contradict any claims of~\cite{madry2017towards}, but simply shows that using the overpowered attack allows us to discover adversarial examples that lay outside of but close to the natural test set.}
% \begin{figure}[ht!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/madry_attack.png}
% 	\caption{An example of a pair of adversarial examples generated by the overpowered attack against the robust classifier trained by~\cite{madry2017towards}. The original image is a 2, as is the encoded image, but the adversarially perturbed image is classified as a 6.}
% 	\label{figure:madry attack}
% \end{figure}
% An important avenue for future work is to identify whether these new attack images can be exploited for more robust models, or studied to understand the limits of adversarial training.

==> experiments_classifier_attacks.tex <==
Most methods to construct adversarial examples try to find perturbations that have small $\ell_p$ norm. First-order attacks on the full system are intractable to generate; in this section, we demonstrate robustness to first-order attacks on the unprotected classifier. 

We first focus on the case where the adversarial perturbation has low $\ell_\infty$ norm, where we use the Fast Gradient Sign~\cite{goodfellow2014explaining} method. We perform \textit{untargeted attacks}---we only require that the classifier predicts some label other than the true label; the adversarial perturbation is given by
\begin{equation}\label{eq: adversarial perturbation}
\delta=+\epsilon \cdot \text{sign}(\nabla_X L(y,C_\theta(X))|_{X=x}),
\end{equation}
where $x$ is the original image and $y$ is its label; $L(y;C_\theta(x))$ is the cross entropy loss between the label $y$ and the prediction on $x$. For the CelebA dataset, we additionally evaluated how robust Invert-and-Classify is against the Carlini-Wagner $\ell_2,\,\ell_0,\,\ell_\infty$ attacks~\citep{carlini2017towards}. For the $\ell_2$ attack, we set the confidence parameter to 5.

%\paragraph{MNIST}
%\subsubsection*{Quantitative Results}
\textbf{MNIST:} The accuracy of the MNIST classifier and Invert-and-Classify defense for varying $\epsilon$ is shown in Figure \ref{figure: mnist classifier attack bar plot}.
\textbf{CelebA:} We report the accuracy of the CelebA classifier with Invert-and-Classify against the FGSM attack and Carlini-Wagner attacks in Table \ref{table: celeba classifier attack}. Figure~\ref{figure: celebA defense qualitative} shows the reconstructions obtained by Invert-and-Classify for women and men in the CelebA dataset.
\begin{figure}[ht]
	\centering
	\includegraphics[width=0.4\columnwidth]{line_plot_accuracy_nodefense_INC.pdf}
	\caption{Accuracy of the classifier and INC protected classifier as we vary the $\ell_{\infty}$ norm of the adversarial perturbation for \textbf{MNIST} using a FGSM attack. }
	\label{figure: mnist classifier attack bar plot}
\end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=0.7\textwidth]{reconstruction_loss}
% 	\caption{This figure plots the $\ell_2$ norm of difference between the input and reconstructed image. $x$ refers to the original image, $x_{adv}=x+\Delta$ is the adversarial example. $z^*=\argmin_z\|x-G(z)\|_2$ is the inverse of $x$, and $z_{adv}^*=\argmin_z\|x_{adv}-G(z)\|_2$ is the inverse of $x_{adv}$. $G(E(x))$ is the result when $x$ is autoencoded by the VAE, while $G(E(x_{adv}))$ is the result when $x_{adv}$ is autoencoded by the VAE. Notice that a high $\ell_2$ error can be used to detect whether an image is adversarial or not.}
% 	\label{figure: reconstruction loss mnist}
% \end{figure}

%\paragraph{CelebA}
%\subsubsection*{Quantitative Results}

\begin{table}[]
\centering
	\caption{Accuracy of the \textbf{celebA} classifier with Invert-and-Classify under different attacks: FGSM~\cite{goodfellow2014explaining} at various powers $\epsilon$, and the ~\citet{carlini2017towards} attacks.}
    \label{table:cla_acc}
  \begin{tabular}{@{}cccc@{}}
    \toprule
    
    \textbf{$\epsilon$} & \phantom{x} & \textbf{No Defense} & \textbf{Invert and Classify} \\
    \midrule
    Clean Data && 97\% & 84\% \\
    FGSM ($\epsilon = 0.05$) && 1\% & 82\% \\
    FGSM ($\epsilon = 0.1$) && 0\% & 80\% \\
    FGSM ($\epsilon = 0.2$) && 0\% & 73\% \\
    Carlini-Wagner $\ell_2$ && 0\% & 77\% \\
    Carlini-Wagner $\ell_0$ && 0\% & 65\% \\
    Carlini-Wagner $\ell_\infty$ && 0\% & 66\% \\
    \bottomrule
  \end{tabular}
\end{table}

%\begin{table}[t]
%\begin{center}
%	\begin{tabular}{|c|cc|}
%		\hline 
%		Attack &  No defense & Invert and Classify \\ 
%		\hline
%		Carlini-Wagner $\ell_2$ & 0\% & 77\% \\
%		Carlini-Wagner $\ell_0$ & 0\%  & 65\%\\ 
%		Carlini-Wagner $\ell_\infty$ & 0\% & 66\% \\
%		\hline
%		\end{tabular}
%		\end{center}
%		\caption{Accuracy of the CelebA classifier and the Invert-and-Classify method against the Carlini-Wagner attacks~\citep{carlini2017towards}. Invert-and-Classify refers to the strategy in Section \ref{subsec: inc implementation}.}
%        \label{table: celeba classifier attack CW}
%\end{table}

%\subsubsection*{Qualitative Results}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{women_defense}
\includegraphics[width=0.45\textwidth]{men_defense}
	\caption{
	In this figure, 
	$x$ are the original images, $G(z^*)$ are the images obtained by inverting $x$, $x_{adv}$ are the adversarial examples obtained from $x$ ($\epsilon = 0.05$), and $G(z_{adv}^*)$ are the images obtained by inverting $x_{adv}$. The values at the corner of each image indicate the confidence with which the classifier predicts the image as the correct gender. 
	As shown, the unprotected gender classifier has confidence $0-8\%$ and the INC protected one confidence $99\%$.
	}
	%\label{figure: celebA women defense qualitative}
	\label{figure: celebA defense qualitative}
	\end{figure}
	
%\begin{figure}[t]
%	\centering
%	\includegraphics[width=0.5\textwidth]{men_defense}
%	\caption{Similar example for male images:  $x$ are the original images, $G(z^*)$ are the images obtained by inverting $x$, $x_{adv}$ are the adversarial examples obtained from $x$ (the adversarial perturbation has $\epsilon = 0.05$), and $G(z_{adv}^*)$ are the images obtained by inverting $x_{adv}$. The values at the bottom right corner of each image indicate the confidence with which the classifier predicts the image as female. 
%	As shown, the unprotected gender classifier has confidence $0-8\%$ and the INC protected one confidence $99\%$.}
%	\label{figure: celebA men defense qualitative}
%\end{figure}

